A multi-centre polyp detection and segmentation dataset for generalisability assessment

Polyps in the colon are widely known cancer precursors identified by colonoscopy. Whilst most polyps are benign, the polyp's number, size and surface structure are linked to the risk of colon cancer. Several methods have been developed to automate polyp detection and segmentation. However, the main issue is that they are not tested rigorously on a large multicentre purpose-built dataset, one reason being the lack of a comprehensive public dataset. As a result, the developed methods may not generalise to different population datasets. To this extent, we have curated a dataset from six unique centres incorporating more than 300 patients. The dataset includes both single frame and sequence data with 3762 annotated polyp labels with precise delineation of polyp boundaries verified by six senior gastroenterologists. To our knowledge, this is the most comprehensive detection and pixel-level segmentation dataset (referred to as \textit{PolypGen}) curated by a team of computational scientists and expert gastroenterologists. The paper provides insight into data construction and annotation strategies, quality assurance, and technical validation. Our dataset can be downloaded from \url{ https://doi.org/10.7303/syn26376615}.

==> supplementaryMaterial.tex <==
%
\section*{Supplementary material}
%
% TODO: sequence color mistaken with single frame color
\setcounter{figure}{0}  
\begin{figure}[t!h!]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/TSNE_positive.pdf}
    \caption{\textbf{t-SNE plot for positive samples:} 2D t-SNE embedding of the ``PolypGen'' dataset based on deep autoencoder extracted features. Each point is an image in the positive samples of the dataset. For each of the 7 boxed regions (dashed black lines) 25 images were randomly sampled for display in a $5\times 5$ image grid. Here, for the 1st and the 7th boxed regions represent mostly the sequence data. Interestingly, the 3rd and the 6th boxed regions mostly represent both polyp and non-polyp data from different provided sequences but belonging to mostly same patient. Similarly, the remaining box areas illustrate the diverse image samples.}
    \label{fig:supplementary_1}
\end{figure}
%
\begin{figure}[t!h!]
    \centering
    \includegraphics[width=0.78\textwidth]{figs/SelectedFrames_Seg_det_C1-C6_PolypGen.pdf}
    \caption{\textbf{Sample polyp annotations from each center:} Segmentation area with boundaries and corresponding bounding box/boxes overlaid images from all six centers. Samples include both small sized polyp ($<10000 pixels$) including some flat polyp samples to large sized ($\geq 40000 pixels$) polyps and polyps during resection procedure such as polyps with blue dyes.}
    \label{fig:supplementary_2}
\end{figure}
%TODO: Ask Thomas to correct the caption!

==> takeout.tex <==
@ARTICLE{Figueredo:2009dg,
   author = {Figueredo, A.~J. and Wolf, P. S.~A.},
   title = {Assortative pairing and life history strategy -- a cross-cultural study},
   journal = {Human Nature},
   volume = {20},
   pages = {317-330},
   year = {2009},
   doi = {https://doi.org/10.1007/s12110-009-9068-2}
}

@MISC{Hao:gidmaps:2014,
  author = {Hao, Z. and AghaKouchak, A. and Nakhjiri, N. and Farahmand, A},
  year = {2014},
  title = {Global integrated drought monitoring and prediction system ({GIDMaPS}) data sets},
  howpublished = {\emph{figshare} \url{https://doi.org/10.6084/m9.figshare.853801}}
}

@Book{behringer2014manipulating,
 author = {Behringer, Richard},
 title = {Manipulating the mouse embryo: a laboratory manual},
 publisher = {Cold Spring Harbor Laboratory Press},
 year = {2014},
 address = {New York},
 isbn = {978-1-936113-01-9}
 }
 
 
 
 @article{haggar2009colorectal,
  title={Colorectal cancer epidemiology: incidence, mortality, survival, and risk factors},
  author={Haggar, Fatima A and Boushey, Robin P},
  journal={Clinics in colon and rectal surgery},
  volume={22},
  number={4},
  pages={191},
  year={2009},
  publisher={Thieme Medical Publishers}
}

@article{Holme2013flexible,
  title={Flexible sigmoidoscopy versus faecal occult blood testing for colorectal cancer screening in asymptomatic individuals},
  author={Holme, {\O}yvind and Bretthauer, Michael and Fretheim, Atle and Odgaard-Jensen, Jan and Hoff, Geir},
  journal={The Cochrane Library},
  year={2013},
  publisher={Wiley Online Library}
}

@article{von2012european,
  title={European guidelines for quality assurance in colorectal cancer screening and diagnosis. --Executive summary},
  author={Von Karsa, L and Patnick, J and Segnan, N},
  journal={Endoscopy},
  volume={44},
  number={S 03},
  pages={SE1--SE8},
  year={2012},
  publisher={{\copyright} Georg Thieme Verlag KG}
}

@article{geetha2017heuristic,
author = {K, Geetha and C, Rajan},
doi = {10.22034/APJCP.2017.18.6.1681},
file = {::},
issn = {2476-762X},
journal = {Asian Pacific journal of cancer prevention : APJCP},
keywords = {Colon cancer,Colonoscopy,Polyps,Segmentation,Video Capsule Endoscopy,binary pattern},
number = {6},
pages = {1681--1688},
pmid = {28670889},
title = {{Heuristic Classifier for Observe Accuracy of Cancer Polyp Using Video Capsule Endoscopy}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/28670889},
volume = {18},
year = {2017}
}

@article{quintero2012progress,
  title={Progress and challenges in colorectal cancer screening},
  author={Quintero, Enrique and Hassan, Cesare and Senore, Carlo and Saito, Yutaka},
  journal={Gastroenterology research and practice},
  volume={2012},
  year={2012},
  publisher={Hindawi}
}

@article{rex2002rationale,
  title={Rationale for colonoscopy screening and estimated effectiveness in clinical practice.},
  author={Rex, Douglas K},
  journal={Gastrointestinal endoscopy clinics of North America},
  volume={12},
  number={1},
  pages={65--75},
  year={2002}
}

@article{lieberman2005quality,
  title={Quality and colonoscopy: a new imperative},
  author={Lieberman, David},
  journal={Gastrointestinal endoscopy},
  volume={61},
  number={3},
  pages={392--394},
  year={2005},
  publisher={Elsevier}
}


@article{pabby2005analysis,
  title={Analysis of colorectal cancer occurrence during surveillance colonoscopy in the dietary Polyp Prevention Trial},
  author={Pabby, Ajay and Schoen, Robert E and Weissfeld, Joel L and Burt, Randall and Kikendall, James W and Lance, Peter and Shike, Moshe and Lanza, Elaine and Schatzkin, Arthur},
  journal={Gastrointestinal endoscopy},
  volume={61},
  number={3},
  pages={385--391},
  year={2005},
  publisher={Elsevier}
}

@article{rex2002quality,
  title={Quality in the technical performance of colonoscopy and the continuous quality improvement process for colonoscopy: recommendations of the US Multi-Society Task Force on Colorectal Cancer},
  author={Rex, Douglas K and Bond, John H and Winawer, Sidney and Levin, Theodore R and Burt, Randall W and Johnson, David A and Kirk, Lynne M and Litlin, Scott and Lieberman, David A and Waye, Jerome D and others},
  journal={The American journal of gastroenterology},
  volume={97},
  number={6},
  pages={1296},
  year={2002},
  publisher={Nature Publishing Group}
}

@article{wang2015polyp,
  title={Polyp-alert: Near real-time feedback during colonoscopy},
  author={Wang, Yi and Tavanapong, Wallapak and Wong, Johnny and Oh, Jung Hwan and De Groen, Piet C},
  journal={Computer methods and programs in biomedicine},
  volume={120},
  number={3},
  pages={164--179},
  year={2015},
  publisher={Elsevier}
}

@article{iddan2000wireless,
  title={Wireless capsule endoscopy},
  author={Iddan, Gavriel and Meron, Gavriel and Glukhovsky, Arkady and Swain, Paul},
  journal={Nature},
  volume={405},
  number={6785},
  pages={417},
  year={2000},
  publisher={Nature Publishing Group}
}

@inproceedings{cui2010bleeding,
  title={Bleeding detection in wireless capsule endoscopy images by support vector classifier},
  author={Cui, Lei and Hu, Chao and Zou, Yuexian and Meng, Max Q-H},
  booktitle={Information and Automation (ICIA), 2010 IEEE International Conference on},
  pages={1746--1751},
  year={2010},
  organization={IEEE}
}


% 		KvasirCapsule-SEG~\cite{jha2021nanonet} & Polyps$^\diamond$ & 55 images$^\dag$&  open academic\\ \hline %$^\diamond$

% 	Only dataset please -- no challenge especially if they are subset of these datasets, I leave Capsule and Kvasir-SEG	
% 		\shortstack{Medico automatic polyp\\ segmentation challenge~\cite{jha2020medico}} & Polyps & 160 images$^\dag$$^\theta$ &  open academic \\ \hline
		
% 		EndoTect 2020 Challenge~\cite{hicks2020endotect}& Polyps & 200 images$^\dag$$^\theta$ &open academic \\ \hline
